Physics potential of the International Axion Observatory (IAXO)

We review the physics potential of a next generation search for solar axions: the International Axion Observatory (IAXO). Endowed with a sensitivity to discover axion-like particles (ALPs) with a coupling to photons as small as $g_{a\gamma}\sim 10^{-12}$ GeV$^{-1}$, or to electrons $g_{ae}\sim$10$^{-13}$, IAXO has the potential to find the QCD axion in the 1 meV$\sim$1 eV mass range where it solves the strong CP problem, can account for the cold dark matter of the Universe and be responsible for the anomalous cooling observed in a number of stellar systems. At the same time, IAXO will have enough sensitivity to detect lower mass axions invoked to explain: 1) the origin of the anomalous "transparency" of the Universe to gamma-rays, 2) the observed soft X-ray excess from galaxy clusters or 3) some inflationary models. In addition, we review string theory axions with parameters accessible by IAXO and discuss their potential role in cosmology as Dark Matter and Dark Radiation as well as their connections to the above mentioned conundrums.

==> sections/aprdnbe.tex <==
\begin{figure}[t] \centering
%%%%%\psfrag{Shielding}{Shielding}
%%%%%\includegraphics[width=5cm]{magnet1.eps}
%\includegraphics[width=\textwidth]{pics/sketch_helioscope}\hspace{2pc}%
\caption{\label{fig:NGAH_sketch} Conceptual arrangement
of an enhanced axion helioscope with X-ray focalization. Solar axions are converted into photons by the transverse magnetic field inside the bore of a powerful magnet. The resulting quasi-parallel beam of photons of cross sectional area $A$ is concentrated by an appropriate X-ray optics onto a small spot area $a$ in a low background detector. The envisaged design for IAXO, shown in Figure~\ref{fig:IAXO_sketch}, includes eight such magnet bores, with their respective optics and detectors. }
\end{figure}


The International Axion Observatory (IAXO) is a next generation axion helioscope that aims at a substantial step forward, of more than one order of magnitude, in sensitivity to $\gagamma$ with respect to current best limits. The baseline layout of the experiment is based on the enhanced axion helioscope studied in~\cite{Irastorza:2011gs} and sketched in Figure~\ref{fig:NGAH_sketch}. In this configuration the entire cross sectional area of the magnet is equipped with X-ray focusing optics to increase the signal-to-noise ratio. When the magnet is pointing to the Sun, solar axions are converted into photons, that are  focused and detected by low background X-ray detectors placed at the focal point of the telescopes. In this way a larger magnet aperture $A$ translates directly into the figure of merit of the experiment, as a larger signal is expected while the detector background remains low. This opens the way for new large-volume magnet configurations, like the ones of superconducting \textit{detector} magnets typically developed for high energy physics.

A useful figure of merit (FOM) was introduced in~\cite{Irastorza:2011gs} to easily gauge the relative importance of the various experimental parameters affecting the sensitivity of a helioscope:

\begin{equation}
f \equiv  f_M \: f_{DO} \:f_T
\end{equation}
where we have factored the FOM to explicitly show the contributions from various experimental subsystems: magnet, detectors and optics, and tracking (effective exposure time of
the experiment)
\begin{equation} \label{eq:foms}
f_M  = B^2\:L^2\:A \;\;\;\;\;\; f_{DO}=\frac{\epsilon_d \:
\epsilon_o}{\sqrt{b\:a}} \:\:\:\:\:\: f_T=\sqrt{\epsilon_t\:t} \ .
\end{equation}


%\begin{equation}
%\gagamma^4 \sim B^2 L^2 A \; \epsilon_d b^{-1/2} \; \epsilon_o a^{-1/2} \; \epsilon_t^{1/2} t^{1/2}
%\end{equation}

\noindent where $B$, $L$ and $A$ are the magnet field, length and
cross sectional area, respectively. The efficiency $\epsilon =
\epsilon_d \: \epsilon_o \: \epsilon_t$, being $\epsilon_d$ the
detectors' efficiency, $\epsilon_o$ the optics throughput or
focusing efficiency (it is assumed that the optics covers the
entire area $A$), and $\epsilon_t$ the data-taking efficiency,
i.~e.~the fraction of time the magnet tracks the Sun (a parameter
that depends on the extent of the platform movements). Finally,
$b$ is the normalized (in area and time) background of the
detector,  $a$ the total focusing spot area and $t$ the duration
of the data taking campaign.

Following this metric, IAXO thus aims at a  $f$ more than a factor 10$^4$ larger that its predecessor CAST. We have recently finished a conceptual design report (CDR) of the experiment~\cite{Armengaud:2014gea,Irastorza:1567109}, demonstrating the technical feasibility of this step in sensitivity, and whose main parameters will be reviewed below. Previous implementations of axion helioscopes have relied on existing equipment that were originally built for other experimental purposes. On the contrary, IAXO subsystems (magnet, optics and detectors) are entirely conceived and optimized for solar axion detection. The design prescriptions have been to rely on state-of-the-art technologies scaled up within realistic limits, i.e. no R\&D is needed to reach the stated experimental parameters. The \textit{baseline} sensitivity projections studied below will refer to the experimental parameters anticipated in the CDR. More recently, the realization of an intermediate experimental stage, BabyIAXO, featuring a scaled-down prototype version of the magnet, optics and detectors, is being considered. This new activity brings the opportunity to explore potential improvements over the CDR figure of merit of the full infrastructure, potentially resulting on an \textit{upgraded} sensitivity scenario for IAXO. The sensitivity projections shown below and in the plots all throughout this paper refer to these three experimental scenarios: BabyIAXO, IAXO-baseline and IAXO-upgraded. The experimental parameters corresponding to each of them are listed in table~\ref{tab:scenarios}, and the prescriptions to define them are discussed in the following.

%All axion helioscopes to date have made use of ``recycled'' magnets that were originally built for other experimental purposes. The CAST success has relied, to a large extent, on the availability of the first-class LHC test magnet. Going substantially beyond CAST sensitivity is possible only by going to a new magnet, designed and built maximizing the helioscope magnet's figure of merit $f_M  = B^2\:L^2\:A$, where $B$, $L$ and $A$ are the magnet's field strength, length and cross sectional area, respectively. $f_M$ is defined proportional to the photon signal from converted axions. Improving CAST $f_M$ can only be achieved~\cite{Irastorza:2011gs} by a completely different magnet configuration with a much larger magnet aperture $A$, which in the case of the CAST magnet is only $3\times10^{-3}$~m$^2$. However, for this figure of merit to directly translate into signal-to-noise ratio of the overall experiment, the entire cross sectional area of the magnet must be equipped with X-ray focusing optics. The layout of this \textit{enhanced axion helioscope}, sketched in Figure \ref{fig:NGAH_sketch}, was proposed in~\cite{Irastorza:2011gs} as the basis for IAXO.

\begin{figure}[!t]
\begin{center}
%    \includegraphics[width=0.8\textwidth] {pics/system_wo_dome.jpg}
    \caption{Schematic view of IAXO. Shown are the cryostat, eight telescopes+detector lines, the flexible lines guiding services into the magnet, cryogenics and powering services units, inclination system and the rotating platform for horizontal movement. The dimensions of the system can be appreciated by a comparison to the human figure positioned by the rotating table~\cite{Armengaud:2014gea}.}
    \label{fig:IAXO_sketch}
\end{center}
\end{figure}


The central component of IAXO is therefore a large superconducting magnet. Contrary to previous helioscopes, IAXO's magnet will follow a toroidal multibore configuration~\cite{Shilon:2012te}, to efficiently produce an intense magnetic field over a large volume. The baseline layout of the IAXO magnet is a 25 m long and 5.2 m diameter toroid assembled from 8 coils, and generating effectively 2.5 T average (5 T maximum) in 8 bores of 600 mm diameter.
%This represents a 300 times better $f_M$ than CAST magnet.
The toroid's stored energy is 500 MJ. The design is inspired by the ATLAS barrel and end-cap toroids~\cite{tenKate:1158687,tenKate:1169275}, the largest superconducting toroids built and presently in operation at CERN. The superconductor used is a NbTi/Cu based Rutherford cable co-extruded with Aluminum, a successful technology common to most modern detector magnets. Figure~\ref{fig:IAXO_sketch} shows the conceptual design of the overall infrastructure~\cite{Armengaud:2014gea}. IAXO needs to track the Sun for the longest possible period. For the rotation around the two axes to happen, the 250 tons magnet is supported at the centre of mass by a system also used for very large telescopes. The necessary magnet services for vacuum, helium supply, current and controls are rotating along with the magnet.

Each of the eight magnet bores is equipped with X-ray telescopes that rely on the high X-ray reflectivity on multi-layer surfaces at grazing angles. By means of nesting, that is, placing concentric co-focal X-ray mirrors inside one another, large surface of high-throughput optics can be built. The IAXO collaboration envisions using optics similar to those used on NASA's NuSTAR~\cite{nustar2013}, an X-ray astrophysics satellite with two focusing telescopes that operate in the 3 - 79 keV band.  The NuSTAR's optics, shown in Figure~\ref{fig:IAXO_optic}, consists of thousands of thermally-formed glass substrates deposited with multilayer coatings to enhance the reflectivity above 10 keV.  For IAXO, the mirror arrangement and coatings are designed to match the solar axion spectrum. The conceptual design of the IAXO telescopes~\cite{doi:10.1117/12.2024476} can be seen on the right of Figure~\ref{fig:IAXO_optic}. As proven in~\cite{Armengaud:2014gea,Irastorza:1567109,doi:10.1117/12.2024476}, this technology can equip the aperture area of IAXO magnet bores with focalization efficiency of around 0.6 and focal spot areas of about 0.2 cm$^2$.




%Another area for improvement will be the x-ray optics. Although CAST has proven the concept, only one of the four CAST magnet bores is equipped with optics. Each of the eight IAXO magnet bores will be equipped with By working at shallow incident angles, it is possible to make mirrors with high reflectivity. Here the challenge is not so much achieving exquisite focusing or near-unity reflectivity, but the availability of cost-effective x-ray optics of the required size. For nearly 50 years, the x-ray astronomy and astrophysics community has been building telescopes following the design principle of Hans Wolter, employing two conic-shaped mirrors to provide true-imaging optics.  This class of optics allows ``nesting'', that is, placing concentric co-focal x-ray mirrors inside one another to achieve high throughput. The IAXO collaboration envisions using optics similar to those used on NASA's NuSTAR~\cite{nustar2013}, an x-ray astrophysics satellite with two focusing telescopes that operate in the 3 - 79 keV band.  The NuSTAR's optics, shown in Figure~\ref{fig:IAXO_optic_det}, consists of thousands of thermally-formed glass substrates deposited with multilayer coatings to enhance the reflectivity above 10 keV (figure 2).  For IAXO, the multilayer coatings will be designed to match the solar axion spectrum~\cite{doi:10.1117/12.2024476}.

\begin{figure}[!b]
\begin{center}
%    \raisebox{-.5\height}{\includegraphics[width=7cm] {pics/nustar.jpg}}
%    \raisebox{-.5\height}{\includegraphics[width=8cm] {pics/optic.pdf}}
    \caption{Left: the NuSTAR X-ray telescope, with optics very similar to that proposed for IAXO.  Right: conceptual design of the X-ray optics needed for IAXO.}
    \label{fig:IAXO_optic}
\end{center}
\end{figure}


At the focal plane in each of the optics, IAXO will have low-background X-ray  detectors. The baseline technology for these detectors are small gaseous chambers read by pixelated planes of micro-mesh gas structure (Micromegas)~\cite{Giomataris:1995fq}. These detectors have been successfully used and developed in CAST and other low background applications~\cite{Abbon:2007ug}. The latest CAST detectors have achieved background levels below $10^{-6}$ \ckcs\ with prospect for improvement down to $10^{-7}$ or even $10^{-8}$ \ckcs\ ~\cite{Aune:2013nza}.  These background levels are achieved by the use of radiopure detector components, appropriate shielding, and offline discrimination-algorithms on the 3D event topology in the gas registered by the pixelised readout. A pathfinder system combining an X-ray optics of the same type as proposed for IAXO and a Micromegas detector has been operated in CAST during 2014 and 2015 with the expected performance~\cite{Aznar:2015iia}. Alternative or additional technologies are being considered to complement the capabilities of Micromegas detectors or to extent them in specific aspects. Low noise CCDs are  being actively developed for WIMP dark matter searches and could potentially obtain background levels low enough for IAXO~\cite{Barreto:2011zu}. Ingrid detectors, similar to Micromegas detectors but built on a small CMOS pixelized readout~\cite{Krieger:2014wxa}, enjoy very low energy threshold down to the tens of eV, and thus are of interest for the search of specific solar axion production channels lying at lower energies, like the ones mediated by the axion-electron coupling. Also of interest for the latter are magnetic metallic calorimeters (MMC)~\cite{Ranitzsch2012}, enjoying much lower energy threshold and energy resolution, and whose low-background capabilities are being studied. Low energy threshold and resolution are also of interest to extract precise $m_a$-dependent spectral information from a possible signal. Even if helioscopes bounds are conventionally considered mass-independent (if not using buffer gas) below the coherence limit, for $m_a$ values close to the coherence condition $qL \sim 1$ the expected signal shows a slight deviation at low energies. For some ranges of $m_a$ and $\gagamma$ this can be used to effectively determine $m_a$ with some precision~\cite{massdet_preparation}. [Extend this to a small section?]



\begin{figure}[t]
\begin{center}
%\includegraphics[height=8cm] {pics/BabyIAXO.jpg}
    \caption{Conceptual design of BabyIAXO}
 \label{fig:babyiaxo}
\end{center}
\end{figure}

The values for everyone of these parameters are listed in table~\ref{tab:scenarios} for three different scenarios. The column labeled \textit{IAXO baseline} shows the set of values anticipated in our CDR for IAXO, and are considered a realistic estimation within current state of the art. We refer to~\cite{Armengaud:2014gea} for a careful justification of those values. However, we now envision, as a first step, the realization of an intermediate stage, called BabyIAXO, featuring a scaled-down prototype magnet, as well as prototype optics and detectors, all representative of the final systems. BabyIAXO will serve as a testbed for all technologies in the full IAXO, but at the same time will deliver competitive physics. The BabyIAXO magnet is preliminarily conceived as a 10-m long, single-bore magnet, with magnetic field strength similar to that of the full IAXO magnet described above. The diameter of the bore will be 60~cm and will be equipped with one single detection line, optics and detector, of equal dimensions than the final IAXO systems. The magnet design differs slightly from the CDR design, in that the conductor is distributed around the bore following a saddle dipole design. This somewhat less conservative arrangement takes advantage of the realization of an intermediate prototype to mitigate risks and explore improvements in the magnet figure of merit. This design allows for a more efficient use of the conductor, and the magnetic field is more homogeneous across the magnet bore, which should result in a comparatively lower peak field and, in principle, larger margin to possibly go to higher fields. A technical description of BabyIAXO magnet will be object of another dedicated publication. Figure~\ref{fig:babyiaxo} shows a conceptual design of the BabyIAXO setup, whose expected experimental parameters are listed in the first column of table~\ref{tab:scenarios}. For all non-magnet parameters, our CDR listed two set of values, one more conservative and one more optimistic. In this work we have assigned the latter to the IAXO baseline scenario, with the justification that the BabyIAXO stage will facilitate to achieve them in the final IAXO, while the former are assigned to the BabyIAXO set of values.




In addition, the experience with BabyIAXO is expected to test enhanced design choices that eventually lead to improved IAXO FOM values, especially $f_M$, beyond the ones anticipated in our CDR. The column labeled \textit{IAXO upgraded} represent this possible improved scenario. Collectively they constitute a factor $\sim$10 better $f$ (of which a factor 4 better $f_M$) that the baseline scenario. However, the extent to which those possible improvement may eventually realized is tentative, and this scenario must be considered as a desirable target which feasibility will be studied as part of the BabyIAXO stage.

\begin{table}[!b]
\footnotesize
\centering
\begin{tabular}{ccccc}
\hline  \textbf{Parameter} & \textbf{Units} & \textbf{ BabyIAXO} & \textbf{IAXO baseline }  & \textbf{IAXO upgraded }\\
\hline \\
 $B$           & T         & 2.5       & 2.5  & 3.5        \\
 $L$           & m         & 10       & 20    & 22    \\
 $A$           & m$^2$    & 0.28  & 2.3  & 3.9  \\
                                                                    \\
\hline
 $f_M^*$         &           & 10              & 300     & 1200 \\
                                                    \\

 $b$             & ${\rm keV^{-1}\, cm^{-2}\, s^{-1}}$ &  $5\times10^{-8}$ & $10^{-8}$& $10^{-9}$\\
 $\epsilon_d$  &              & 0.7      & 0.8 & 0.8   \\
 $\epsilon_o$  &              & 0.5      & 0.7 & 0.7   \\
 $a$             &  cm$^{2}$    &  8 $\times$ 0.2   & 8 $\times$ 0.15  & 8 $\times$ 0.15  \\
 %\hline
 %$f_{DO}^*$      &              & 17   & 60      \\
                                                                        \\
 $\epsilon_t$  &                     & 0.5   & 0.5  & 0.5  \\
 $t$             & year                    & 3     & 3 & 5    \\
 %\hline
 %$f_T^*$         &           & 1                    & 3.5     & 3.5     \\                                                                        \\
 %\hline
 %$f^*$           &           & 1               & $2 \times 10^4$      & $6 \times 10^4$     \\
 \hline \hline
\end{tabular}
\caption{Values of the relevant experimental
parameters representative of BabyIAXO as well as IAXO, both the \textit{baseine} and \textit{upgraded} scenarios, based on the considerations explained in the text.}\label{tab:scenarios}
\end{table}




%CAST has enjoyed the sustained development of its detectors towards lower backgrounds during its lifetime. The latest generation of Micromegas detectors in CAST are achieving backgrounds below $\sim$$10^{-6}$~\ckcs~~\cite{Aune:2013pna,Aune:2013nza}. This value is already a factor of more than 100 better than the background levels obtained during the first data-taking periods of CAST. Prospects for reducing this level to $10^{-7}$ \ckcs\ or even lower appear feasible after the active R\&D going on, in particular that being carried out at the University of Zaragoza, under the T-REX ERC-funded project~\cite{Irastorza2011_EAS,Dafni:2012fi,Dafni:2012zz,trexwebpage}. As part of this work, a replica of the CAST Micromegas detectors is taking data in an underground test bench at the Laboratorio Subterráneo de Canfranc, already reaching a background level of $\sim$$10^{-7}$~\ckcs~~\cite{Aune:2013pna}. These background levels are achieved by the use of radiopure detector components, appropriate shielding, and offline discrimination-algorithms on the 3D event topology in the gas registered by the pixelised readout.





%
%
%\begin{figure}[!b]
%\begin{center}
%    \includegraphics[height=5cm] {castshielding.jpg}
%    \includegraphics[height=5cm] {nustar.jpg}
%    \caption{Left: two lead- and copper-shielded, ultra-low background Micromegas x-ray detectors currently in use at CAST. Right: the NuSTAR x-ray telescope, with optics very similar to that proposed for IAXO.}
%    \label{fig:IAXO_optic_det}
%\end{center}
%\end{figure}





%For some of the additional physics cases of IAXO, lowering the theshold well below 1 keV is interesting. For this reason other types of x-ray detection technologies are also under consideration, like GridPix detectors, Transition Edge Sensors (TES) or low noise CCDs to be placed at the optics focal points. Beyond that, because a high magnetic field in a large volume is an essential component in any axion experiment, IAXO could evolve to a generic ``axion facility'' and host different detection techniques. The most relevant of these possibilities, at the moment actively explored, is to use microwave cavities and antennas to search for dark-matter axions. Some of the developments being carried out in the community (briefly mentioned above in section \ref{sec:searches}) could profit from the availability of the large magnetic field of IAXO, and reach sensitivity to axions in mass ranges complementary to those in previous searches.

%The IAXO collaboration has recently finished the conceptual design of the experiment~\cite{Armengaud:2014gea}, and last year a Letter of Intent~\cite{Irastorza:1567109} was submitted to the  SPS and PS experiments Committee (SPSC) of CERN.

%The committee acknowledged the physics goals of IAXO and recommended proceeding with the next stage, the creation of the technical design report (TDR), a necessary step before facing construction. As part of the TDR, prototyping activities are foreseen, including magnet (the construction and test of a single shorter superconducting coil), optics and detector aspects. At the same moment of preparation of this review, a ``IAXO optics+detector pathfinder system'' has just been assembled in CAST at CERN. It consist of a small x-ray optics (of CAST bore dimensions) coupled to a low-background Micromegas detector. This is the first time that the two techniques pioneered by CAST --x-ray focusing and low background detectors--, previously used in different lines of the experiment, are now coupled together in the same line. It is also the first time that an x-ray optics is manufactured specifically for axion physics. This system will tests the two technologies proposed for IAXO coupled together. The first data is already being taken: the experience with this system will be precious for the preparation of IAXO.




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\section{Updated sensitivity plots for IAXO}
%\label{sec:sensitivity}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%\begin{figure}[!b]
%\begin{center}
%    \includegraphics[height=7cm] {CScenarios.pdf}
%    \includegraphics[height=7cm] {IAXOgaaZoom.pdf}
%    \caption{IAXO sensitivity projections, for the three scenarios of table \ref{tab:scenarios}, in the $C_\gamma$-$m_a$ (left) or $\gagamma$-$m_a$ (right) planes. Green lines are specific axion models. }
%%    \label{fig:IAXO_optic_det}
%\end{center}
%\end{figure}


%\begin{figure}[!t]
%\begin{center}
%    \includegraphics[height=7cm] {gaagaevsma.pdf}
%    \includegraphics[height=7cm] {gaavsgae.pdf}
%\caption{IAXO sensitivity projections, for the three scenarios of table \ref{tab:scenarios}, for the axion-electron coupling mediated signal, in the $g_{ae}\gagamma$-$m_a$ (left) and $\gagamma$-$g_{ae}$ (right) planes, the latter for $m_a \lesssim 0.01$.}%    \label{fig:IAXO_optic_det}
%\end{center}
%\end{figure}
%

\begin{figure}[!b]
\begin{center}
%    \includegraphics[height=10cm] {pics/ExclusionPlot.pdf}
%\tikzsetnextfilename{pics/ExclusionPlot}
% \resizebox{0.8\textwidth}{!} {\input{pics/ExclusionPlot.tex}}
    \caption{caption}
    \label{fig:excluion_iaxo}
\end{center}
\end{figure}




The IAXO sensitivity projections shown in Fig.~\ref{fig:excluion_iaxo} as well as in all plots throughout this paper refer to the three scenarios of table~\ref{tab:scenarios}. They have been computed  by means of Monte Carlo simulation of the expected background counts in the optics spot area, computation of the likelihood function and subsequent derivation of the 95\% upper limit on the $\gagamma$ assuming no detected signal. The calculation is repeated for a range of $m_a$ values in order to build full sensitivity lines in the $(\gagamma,m_a)-$plane. For the purpose of this analysis, and following similar prescriptions as in~\cite{Irastorza:1567109}, detector background and efficiency are assumed flat with energy down to arbitrarily low energies. The axion-photon conversion in the magnet is approximated to the conversion in an homogeneous field, and the focusing effect is reduced to the equivalent effect of enhancing the signal-to-noise ratio due to the fact of confining the signal counts into the spot area. For the IAXO baseline and upgraded scenarios, an additional buffer gas data taking phase is considered, giving rise to the extended step-wise sensitivity line at high masses (0.01-0.25 eV). This data taking phase is composed by a number of overlapping gas density steps spanning the desired mass range. While in previous projections~\cite{Irastorza:2011gs} an equal exposure time is assigned to each step, resulting in a exclusion line more or less horizontal in $\gagamma$, in this case the exposure time is different for every step and adjusted to obtain a sensitivity down to the DFSZ $\gagamma$ for every $m_a$ value. Of course different prescriptions to distribute the total exposure time among the steps are possible, depending on the motivation, e.g. to go for larger $m_a$ or lower $\gagamma$. For the sake of simplicity, the BabyIAXO line has been computed as an only vacuum data taking phase, although a gas phase could also be considered.

\subsection{Direct search for DM axions with IAXO and BabyIAXO}

Although the focus of this paper has been the physics potential of IAXO is its baseline configuration as a helioscope, the (Baby)IAXO magnet constitutes a remarkable infrastructure to implement additional setups to search for axions/ALPs in alternative ways. A most appealing option is to implement DM axion detectors that could exploit the particular features of the IAXO magnet. The basic idea of
the axion-haloscope-technique proposed in ~\cite{Sikivie:1983ip} is to
combine a high-$Q$ microwave cavity
inside a magnetic field to trigger the conversion of axions of the DM
halo into photons. A straightforward implementation of this concept in one bore of the IAXO  magnet gives competitive sensitivity~\cite{redondo_patras_2014} even using relatively conservative values for detection parameters, thanks to the large $B^2 V$ available, in the approximate mass range of 0.6 -- 2 $\mu$eV. Another recent concept proposes the use of a carefully placed pick-up coil to sense the small small oscillating magnetic field that could be produced by the DM axion interacting in a large magnetic volume~\cite{Sikivie:2013laa}. This technique is best suited for even lower $m_a$ and is better implemented in toroidal magnets~\cite{Kahn:2016aff,Silva-Feaver:2016qhh}. The large size and toroidal geometry of IAXO suggest that it could host a very competitive version of this detection technique.

However, as can be seen from Fig.\ref{fig:DM_predictions}, there is a strong motivation to explore the mass range for QCD axion DM well above $10^{-5}$~eV.
% is largely unexplored by so-called axion haloscopes.
The difficulty in searching in the ``high-mass'' range can be understood from
the fact that the figure of merit of scanning with haloscopes for axion DM goes
with the square of the cavity volume times the $Q$ factor of the cavity.
Most existing setups use solenoidal magnets and cylindrical
cavities. The diameter of the cylinder sets the frequency scale of the resonance
and thus the axion mass scale which the experiment is sensitive to. Thus going to
high mass means going to small diameters. In addition, the cavity quality factor $Q$ typically decreases for smaller cavities.

To tackle higher masses, different strategies are being developed in the community. For instance, to compensate the loss in $V$ one can go to very strong magnetic fields and/or use superconducting cavities to keep $Q$ large. Another avenue is to decouple $V$ from the resonant frequency and go for large $V$ structures resonating at high frequency. Several strategies in this direction are being explored. One of them, currently being tested
in exploratory set-ups at the CAST experiment at CERN~\cite{Desch:2221945,Fischer:2289074}, employ long rectangular cavities~\cite{Baker:2011na}.
The particular advantage is that the volume can be kept very large (long cavity), while the resonance frequency
can be rather high, through the usage of relatively thin cavities. Given the size of the (Baby)IAXO magnet, it could host a multitude of rectangular cavities.

The implementation of one those concepts in IAXO is under consideration, but is out of the scope of the present paper. It clearly deserves serious study and will be the object of one or more future publications.

